A Robust Spectral Algorithm for Overcomplete Tensor Decomposition

We give a spectral algorithm for decomposing overcomplete order-4 tensors, so long as their components satisfy an algebraic non-degeneracy condition that holds for nearly all (all but an algebraic set of measure $0$) tensors over $(\mathbb{R}^d)^{\otimes 4}$ with rank $n \le d^2$. Our algorithm is robust to adversarial perturbations of bounded spectral norm. Our algorithm is inspired by one which uses the sum-of-squares semidefinite programming hierarchy (Ma, Shi, and Steurer STOC'16, arXiv:1610.01980), and we achieve comparable robustness and overcompleteness guarantees under similar algebraic assumptions. However, our algorithm avoids semidefinite programming and may be implemented as a series of basic linear-algebraic operations. We consequently obtain a much faster running time than semidefinite programming methods: our algorithm runs in time $\tilde O(n^2d^3) \le \tilde O(d^7)$, which is subquadratic in the input size $d^4$ (where we have suppressed factors related to the condition number of the input tensor).

==> content/dictionary-learning.tex <==
\section{Dictionary learning}

The following lemma allows handling of noise that isn't necessarily small in spectral norm, but which has a component that is relatively spectrally small when normalized to the signal term.
This may be useful for analyzing noise models such as in dictionary learning, where much of the noise occurs within the span of the signal components $a_i \ot a_i$.	
\begin{lemma}
	\label[lemma]{dictionary-perturb}
	Suppose $Q \in \R^{D\times D}$ and $\Qish \in \R^{D\times D}$ are both positive-semidefinite matrices of rank $n$.
	Suppose $\Qish - Q = E_1 + E_2$ with $\|Q^{-1/2}E_1 Q^{-1/2}\| \le \eps$ and $E_1 = \Pi_S E_1 \Pi_S$ and $\|Q^{-1}\| \, \|E_2\| \le \eps$, where $\eps \le 1/9$.
	Let $S$ and $\Sish$ be the columnspaces of $Q$ and $\Qish$ respectively.
	Then
	\begin{equation}
	\|\Pi_S-\Pi_{\Sish}\| \le 3\eps
	\end{equation}
	and for any $x \in \R^D$, the following hold:
	\[ \|(Q^{1/2} - \Qish^{1/2})x\| \le 4\eps \|Q^{1/2}x\| + \sqrt{\eps}\|(\Id - \Pi_S)x\|\,,\]
	\[ \|(Q^{-1/2} - \Qish^{-1/2})x\| \le 4\eps \|Q^{-1/2}x\| + 2\sqrt{\eps}\|(\Id - \Pi_S)x\|\,.\]
\end{lemma}
\begin{proof}
That $\|\Pi_S-\Pi_{\Sish}\| \le 3\eps$ follows from \Cref{eigen-perturb} applied on $Q + E_1$, which has the same columnspace as $Q$, and $\Qish$:
We observe by Weyl's inequality~\cite{Weyl1912} that the $n$th eigenvalue of $Q + E_1$ is at least $1-\eps$ times that of $Q$, and since $\|E_2\|$ is bounded by $\eps$ times the $n$th eigenvalue of $Q$, the result follows. 

To show that $\|(Q^{1/2} - \Qish^{1/2})x\| \le 4\eps \|Q^{1/2}x\|$, we let $M = Q + E_1$ and show the intermediate results that $\|(Q^{1/2} - M^{1/2})Q^{-1/2}\| \le \eps$ and $\|(M^{1/2} - \Qish^{1/2})Q^{-1/2}\| \le 3\eps$.
It then follows from triangle inequality that $\|(Q^{1/2} - \Qish^{1/2})Q^{-1/2}y\| \le 4\eps \|y\|$, and by taking $x = Q^{-1/2}y + z$ where $z \perp S$, we find that $\|(Q^{1/2} - \Qish^{1/2})x\| \le 4\eps \|Q^{1/2}x\| + \|\Qish^{1/2}z\| \le 4\eps \|Q^{1/2}x\| + \eps^{1/2}\|(\Id - \Pi_S)x\|$.

To show that $\|(Q^{1/2} - M^{1/2})Q^{-1/2}\| \le 3\eps$, we use the fact that $(1-\eps)Q \preceq M \preceq (1+\eps)Q$, take the square root which preserves the order since all of the matrices are PSD, and then subtract $Q$ from the inequality to find
\[ ((1-\eps)^{1/2} - 1)Q^{1/2} \preceq M^{1/2} - Q^{1/2} \preceq ((1+\eps)^{1/2} - 1)Q^{1/2}\,.\]
Therefore, $\|(Q^{1/2} - M^{1/2})Q^{-1/2}\| \le \eps$.

To show that $\|(M^{1/2} - \Qish^{1/2})Q^{-1/2}\| \le 3\eps$, we start with $-\eps\Id \preceq \|Q^{-1}\|(\Qish - M) \preceq \eps\Id$ and obtain
\[ M - \eps\|Q^{-1}\|^{-1}\Id \preceq \Qish \preceq M + \eps\|Q^{-1}\|^{-1}\Id\,. \]
Using the fact that $\Qish \succeq 0$, we must have $M - \eps\|Q^{-1}\|^{-1}\Pi_S \preceq \Qish$, since $(\Id-\Pi_S)M \preceq 0$.
Then, since $M - \eps\|Q^{-1}\|^{-1}\Pi_S \succeq M - \eps Q \succeq (1-2\eps)M$ is PSD,
\[ (1-2\eps)^{1/2}M^{1/2} \preceq \Qish^{1/2} \preceq (M+\eps\|Q^{-1}\|^{-1}\Id)^{1/2}\,. \]
So, since $(1-2\eps)^{1/2} - 1 \ge -2\eps$ and $(M+\eps\|Q^{-1}\|\Id)^{1/2} \preceq M^{1/2} + \eps^{1/2}\|Q^{-1}\|^{-1/2}(\Id - \Pi_S) + \eps\Pi_S$,
\[ -2\eps M^{1/2} \preceq \Qish^{1/2} - M^{1/2} \preceq \eps^{1/2}\|Q^{-1}\|^{-1/2}(\Id - \Pi_S) + \eps\Pi_S\,. \]
Finally, we showed earlier that $M^{1/2} \preceq(1+\eps)^{1/2}Q^{1/2}$, so that
\[ -3\eps Q^{1/2} \preceq \Qish^{1/2} - M^{1/2} \preceq \eps^{1/2}\|Q^{-1}\|^{-1/2}(\Id - \Pi_S) + \eps\Pi_S\,. \]
Thus, $\|(M^{1/2} - \Qish^{1/2})Q^{-1/2}\| \le 3\eps$.

The argument that $\|(Q^{-1/2} - \Qish^{-1/2})x\| \le 4\eps \|Q^{-1/2}x\|$ proceeds in the same manner, except that we use triangle inequality on $\|\Pi_S-\Qish^{-1/2}\Qish\Qish^{-1/2}\| \le 3\eps$ and $\|\Pi_S - Q^{-1/2}\Qish Q^{-1/2}\| \le \eps$ to show that $\|\Qish^{-1/2} z\| \le 2\sqrt{\eps}\|z\|$ for $z \perp S$.
\end{proof}




